Combining Machine Learning Classifiers for Stock Trading with Effective Feature Extraction

The unpredictability and volatility of the stock market render it challenging to make a substantial profit using any generalised scheme. Many previous studies tried different techniques to build a machine learning model, which can make a significant profit in the US stock market by performing live trading. However, very few studies have focused on the importance of finding the best features for a particular trading period. Our top approach used the performance to narrow down the features from a total of 148 to about 30. Furthermore, the top 25 features were dynamically selected before each time training our machine learning model. It uses ensemble learning with four classifiers: Gaussian Naive Bayes, Decision Tree, Logistic Regression with L1 regularization, and Stochastic Gradient Descent, to decide whether to go long or short on a particular stock. Our best model performed daily trade between July 2011 and January 2019, generating 54.35% profit. Finally, our work showcased that mixtures of weighted classifiers perform better than any individual predictor of making trading decisions in the stock market.

==> core/acknowledgement.tex <==
\section*{Acknowledgement}
Firstly, thanks to our beloved family members to whom I am, and always will be indebted.
\vspace{5mm}
\\
Secondly, to my supervisor Md. Golam Rabiul Alam for all his help and constant support of our endeavours.
\vspace{5mm}
\\
Thirdly, I would like to thank all the faculty members, staff, our peers and other stakeholders related to BRAC University for providing us an environment in which we were able to develop ourselves, learn to our fullest extent and conduct our research properly.\\


==> core/approval.tex <==
\section*{Approval}

The thesis/project titled “Effective Feature Selection for Real-time  Stock Trading in Variable Time-frames  and Multi Criteria Decision Theory based Efficient Stock Portfolio Management” submitted by 
\begin{enumerate}
  \item A. K. M. Amanat Ullah (20166016)
 
 
\end{enumerate}

of Summer, 2021 has been accepted as satisfactory in partial fulfillment of the requirement for the degree of M.Sc. in Computer Science and Engineering on August 23, 2021. 

\vspace{0.5cm}
\textbf{Examining Committee:}

\vspace{1cm}

Supervisor:\\
(Member)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Md. Golam Rabiul Alam, PhD} \\ \centerline{Associate Professor}\\ \centerline{Department of Computer Science and Engineering}\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}

Examiner:\\
(External)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Chowdhury Farhan Ahmed, PhD} \\ \centerline{Professor}\\ \centerline{Department of Computer Science and Engineering }\\ \centerline{University of Dhaka} } \hspace{1cm} 
\end{center}

Examiner:\\
(Internal)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Md. Ashraful Alam, PhD} \\ \centerline{Assistant Professor}\\ \centerline{Department of Computer Science and Engineering }\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}

Examiner:\\
(Internal)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Muhammad Iqbal Hossain, PhD} \\ \centerline{Assistant Professor}\\ \centerline{Department of Computer Science and Engineering }\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}




Program Coordinator:\\
(Member)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Amitabha Chakrabarty, PhD} \\ \centerline{Associate Professor}\\ \centerline{Department of Computer Science and Engineering }\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}


Head of Department:\\
(Chair)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Sadia Hamid Kazi, PhD} \\ \centerline{Chairperson and Associate Professor}\\ \centerline{Department of Computer Science and Engineering }\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}

\pagebreak

==> core/declaration.tex <==
% Following command is used to created grouped signature line for Four Authors
\newcommand*\wildcard[2][6cm]{\vspace{2cm}\parbox{#1}{\hrulefill\par#2}} 

% A "parbox{}{}" is a box whose contents are created in paragraph mode. 
% "hrulefill{} to chance thickness of underline"

\section*{Declaration}

% It is hereby declared that

% \begin{enumerate} % begin{enumerate} function to create numbered list
%   \item The thesis submitted is my/our own original work while completing degree at Brac University.
%   \item The thesis does not contain material previously published or written by a third party, except where this is appropriately cited through full and accurate referencing.
%   \item The thesis does not contain material which has been accepted, or submitted, for any other degree or diploma at a university or other institution.
%   \item We have acknowledged all main sources of help.
% \end{enumerate}
It is hereby declared that

\begin{enumerate} % begin{enumerate} function to create numbered list
  \item The thesis submitted is my/our own original work while completing degree at Brac University.
  \item The thesis does not contain material previously published or written by a third party, except where this is appropriately cited through full and accurate referencing.
  \item The thesis does not contain material which has been accepted, or submitted, for any other degree or diploma at a university or other institution.
  \item We have acknowledged all main sources of help.
\end{enumerate}

\vspace{1cm}
\textbf{Student’s Full Name \& Signature:} % Testbf{} for Bold

\begingroup

    \begin{center}
        \wildcard{\centerline{A. K. M. Amanat Ullah} \\ \centerline{20166016}} % "centerline{}" to center line
        \hspace{2cm} % "hspace{}" for Blank Horizontal space
        % \wildcard{\centerline{ Miftah Uddin Md Ihsan} \\ \centerline{ 17101259} }
        % \wildcard{\centerline{Fahim Imtiaz} \\ \centerline{15201010} }
        \hspace{2cm}
  
    \end{center}

\endgroup


\pagebreak







==> core/dedication.tex <==
\section*{Dedication }
I would like to dedicate this research to my parents who have brought me to this world and nurtured me to become an adult.  

\pagebreak

==> core/ethics_statement.tex <==
\section*{Ethics Statement}
This thesis was carried out in complete compliance with research ethics norms, and the codes and practices set by BRAC University. I have ensured that all our sources have been cited. As the author of this thesis, I take full responsibility for any ethics code violations. 
\newpage
